Anonymizing Masses: Practical Light-weight Anonymity at the Network Level

In an era of pervasive online surveillance, Internet users are in need of better anonymity solutions for online communications without sacrificing performance. Existing overlay anonymity tools, such as the Tor network, suffer from performance limitations and recent proposals to embed anonymity into Internet protocols face fundamental deployment challenges. In this paper, we introduce Practical Anonymity at the NEtwork Level (PANEL), a practical light-weight anonymity solution based on hardware switching. We implement a prototype of PANEL on a high-performance hardware switch (namely, Barefoot Tofino) using P4 network programming language, and examine the validity and performance of the prototype. Based on our empirical results, PANEL achieves 96% of the actual throughput of the switch and adds a low-latency overhead (e.g., 3% overhead in Skype calls), while offering partial deployablility and transparency (i.e., PANEL requires neither client-side nor server-side modifications).

==> paper-01-intro-old.tex <==
\section{Introduction}
\label{intro}
%Following this: http://www.cs.columbia.edu/~hgs/etc/intro-style.html

The state-of-the-art pervasive online surveillance apparatus is capable of recording, aggregating, and analyzing our online communications, allowing business and government agencies to control, monitor, and influence our online interactions~\cite{surv1,surv3}. Even when the communication content is encrypted, the \emph{metadata}, such as Internet addresses and protocol specifications reveal critical information about the communication, which can be exploited by governments and corporations~\cite{nsa,surv}.



Despite their moderate success, popular low-latency anonymity systems today, such as Tor~\cite{tor}, have only been successful at attracting the most privacy-conscious users who are willing to use them despite their poor performance\footnote{ The total number of active Tor users is currently about 3 million users~\cite{tor-metric}, a figure that is far from the number of active Internet users, which is, by even conservative estimates, more than 3 billion users~\cite{interenetUsage}.}. In this paper, we argue that a fundamentally different approach is necessary for the next generation of low-latency anonymity systems that benefits all Internet users.
We propose  \protocolfullsp (\protocol ), a low-latency anonymity protocol which embeds anonymity into the Internet forwarding infrastructure, and is implemented by Autonomous Systems (ASes).

Under the hood, legacy anonymity tools require dedicated infrastructure: a series of overlay proxies to redirect traffic. This infrastructure typically consists of proxy servers run by volunteers, often with no performance guarantees, which causes bandwidth and latency issues~\cite{anonPerformance, torPerformance}.
Our \emph{network-level} approach, on the other hand, obviates the need for a dedicated overlay and provides ubiquitous communication privacy to users by default. Moreover, it mitigates the undesirable scrutiny drawn by the opt-in nature of overlay systems~\cite{pew2}, while creating a critical anonymity mass to thwart surveillance.


%designed to be practical and deployable at the Internet scale, a property that is essential for any anonymity system to be useful, since it requires a critical mass to thwart surveillance.
%~\cite{torinsteadofip, lap, dovetail, hornet, noPhear, enlistingisp, phi}, 

A number of recent proposals have advocated for a similar network-level approach to anonymity~\cite{torinsteadofip, lap, dovetail, hornet,  enlistingisp, phi}. These proposals are not readily applicable to today's Internet. First, some solutions~\cite{hornet,torinsteadofip} modify the Internet routing and forwarding protocols entirely, essentially taking a \emph{clean-slate} design approach~\cite{cleanslate}. For instance, they rely on end-to-end source-controlled routing model and its variants, such as segment routing~\cite{dovetail, hornet, torinsteadofip}, which are still experimental and not ubiquitously deployed~\cite{t0depr, ipv6srh}. 
Second, existing proposals often lack a clear \emph{partial deployment} pathway~\cite{dovetail,hornet}, failing to take into account limitations imposed in the wide area network by different network actors, such as strict header format checking of IP and transport layers by routers and middleboxes~\cite{ipOptionsNotOption,tcpext1}. Finally, while hardware switching fabrics are pervasive in the Internet due to their high performance and port density~\cite{ForwardingMetamorphosis},  all previous proposals are implemented and tested only on \emph{software switches}~\cite{lap, dovetail, hornet,  enlistingisp, phi}, limiting their deployability.


Our contributions in this paper are twofold:

\begin{itemize}
 \item First, we address the compatibility challenge, by identifying different functionalities that Internet service providers aim to achieve, such as incentive-compatible routing, network filtering and security (enforced by network routers, firewalls and other middleboxes) that compete with \protocolsp anonymity objectives, then separate functionalities along tussle boundaries~\cite{tussle}. \protocol, therefore, bridges the gap between futuristic network-level anonymity proposals and current Internet architecture with a partial deployment strategy, by dividing the ASes on the communication path into \protocol-protected \emph{segments} and legacy segments based on Internet Protocol (IP).
ASes in a single \protocolsp segment are at liberty to choose the anonymization method from existing proposals~\cite{torinsteadofip, lap, dovetail, hornet,  enlistingisp, phi} among themselves. However, on the boundary of a \protocolsp segment, designate border routers, referred to as \emph{landmark} routers, transform  packets to standard IP and transport format with fixed size headers and forward these packets to the legacy network on where the path is decided by each hop individually (hop-by-hop routing). 

\item Second, we propose the first anonymity protocol designed for and tested on high performance hardware switching fabric. Our design is based on the idea of \emph{in-network source information rewriting} (discussed in Section~\ref{source-info-rewriting}) and provides session anonymity and unlinkability. Even though the idea itself has been proposed before, we are the first to demonstrate how it can be materialized on high performance hardware switching fabric, using P4~\cite{p4} programming language for our prototype. This enables \protocolsp to provide additional privacy benefits such as hiding path information without any client-side modification at a forwarding rate that is unparalleled compared to existing anonymity proposals\footnote{\protocolsp segments may choose anonymization methods between themselves which require client-side modification. However, this is outside the scope of this paper.}.

\end{itemize}

 
 
 In summary, \protocolsp is the first network-level anonymity solution that combines the following properties:
\begin{itemize}
			\item{ Defines an interface between network-level anonymity systems and legacy IP network, retaining compatibility with both legacy network by maintaining both hop-by-hop routing and packet header compatibility in legacy network.}
			\item { Is designed to run on hardware switches that are widely deployed on the Internet and is implemented in P4~\cite{p4} to target programmable networks for rapid prototyping and testing.}
			\item{ Is transparent to end hosts and does not require client-side (or server-side) modifications.}
\end{itemize}

%Second, many previous approaches require certain primitives (e.g., line-rate encryption~\cite{hornet}) in every router on the Internet. However, these primitives are not available in most routers, especially at the core of the Internet. %a feature that is missing in most routers at the core of the Internet.% Thus, these assumptions lead to a significant barrier to real-world deployment and adoption of these systems. 


%\textbf{Shortcoming of Anonymity Overlays:} 


%Finally, the  development efforts needed to build and configure overlay solutions to work out-of-box are 
%multiplied by the number of platforms supported by an application, further hindering deployment. 
%Recent proposals for next generation of anonymity systems~\cite{lap,hornet} have not seen any real-world deployment either. 

% Thus, it remains open to design a practical anonymity network that operates at the scale of the Internet.
%Recent surveys show a stark gap between privacy expectations of citizens and the level of privacy they believe they are granted, with more than 90\% of American adults having low confidence in companies and government agencies to keep their data private and secure~\cite{pew1}. In response to these demands, privacy enhancing technologies, including anonymity systems, have emerged. Despite  their modest success, however, anonymity solutions on the Internet have long been restricted to the tech savvy and privacy conscious.

%Even since Snowden revelations raised privacy awareness of Internet users and increased the adoption of privacy tools among general public in 2013, The total number of Tor has only seen a twofold increase on average.
%as shown in Figure~\ref{fig:tor-usage}, 



%Moreover, due to the opt-in nature of Tor and other anonymity systems, installing 
%and using them indicates an intent to participate. This is a  differentiating factor 
%for users of such systems and can invite scrutiny which is undesirable from users' 
%perspective~\cite{pew2}. 
%Looking under the hood, we find that existing low-latency 
%anonymity solutions, such as Tor~\cite{tor} often involve, as a fundamental design principle, 
%the idea of \emph{overlay} network functionality, where a number of hosts connected over 
%an underlying network, commonly Internet Protocol (IP), provide anonymity service. 
%Overlay anonymity networks have a number of drawbacks. 
%\begin{figure}
%  \includegraphics[width=0.5\textwidth]{images/userstats-relay-country-all-2012-11-25-2017-02-23-off}
%  \caption{Number of Tor users between November 2012 and February 2017. The surge in the number of users connecting directly to the Tor network in 2013, which might have been due to a Botnet abuse of Tor hidden servers~\protect\cite{torBotnet}, was followed by a plateau in mid 2014, continuing until now.}
%  \label{fig:tor-usage}
%\end{figure}


%-> rewrite or remove
%Individuals are reported to have taken measures to improve their online  privacy~\cite{pew3} and nation states are taking actions to avoid transiting through third party countries suspected of conducting surveillance~\cite{brazilPrivateNetwork}. However, the consensus among security experts is that few individuals will be capable of protecting themselves from surveillance in the coming years~\cite{pew4} and studies of nation state routing structure reveals that efforts to avoid bypassing third party countries are often futile~\cite{routingDetours, nationStateRouting}.

%





We discuss design goals in Section~\ref{sec:des-goals}, present an overview of \protocolsp in Section~\ref{sec:overview} and our design in Section~\ref{sec:sys-design}. The evaluation of our \protocolsp prototype appears in Section~\ref{sec:eval}, followed by a discussion of related work in Section~\ref{sec:related-work} and a discussion of limitations and potential extensions to \protocolsp in Section~\ref{sec:disc}.

%\hcomment{complete this once the paper is done.}


%We have designed \protocolsp with the goal of being compatible with the current Internet architecture and deployable at Internet-scale, based on the following properties. First, \protocolsp is partially deployable and has an incremental deployment plan --- 
%considering a \emph{subset} of ASs that speak PANEL (called landmark ASs), all traffic originating or transiting such landmark ASs is anonymized.
% provides anonymity to all traffic originating or transiting through \emph{landmark} ASs (an AS that speaks \protocol). %Consequently, \protocolsp remains transparent to nonparticipating network devices, including firewalls and middleboxes. 
%Second, \protocolsp is lightweight and can be realized with building blocks already available on commodity network hardware, even at the core of the Internet. Finally, \protocolsp adheres to routing models that are compatible with common practices and incentive structure of network operators, and avoids models such as source-controlled routing.




 
%Furthermore,  \protocolsp uses primitives that already exist in current routers and switches,
 %without weighing down routing protocol routines in the data-plane with cryptographic overhead. 
 %Performing cryptographic operations at line-rate is a feature that is still missing in most packet processing hardwares and solutions relying on it will have a much slower deployment as a result~\cite{lap, hornet}. 
% and  maintains the structure of IP and transport layer packet headers in order to remain transparent to middleboxes~\cite{tracebox}. 
%Finally, we used P4~\cite{p4}, a field reconfigurable, protocol and target independence programming language to prototype \protocol. Even though, our current design can be implemented using legacy OpenFlow~\cite{openflow}, choosing P4 for prototyping allows us to expand beyond the standard OpenFlow in the future.  %This approach paves the way for deployment of our design on SDN-enabled devices. 
%As a result, we can leverage methods in Software Defined Networking (SDN) to manage the state of flows and orchestrate our deployment in a scalable fashion.
%To our knowledge, \protocolsp is the first privacy enhancing solution compatible with SDN technology in the context of inter-domain anonymity (See Section~\ref{related-work}).


%\begin{itemize}
%\item \textbf{Sender Anonymity}: The first order privacy goal of \protocolsp in the first stage, is to hide where flows originate from,  by obfuscating source information. Thus,  \protocolsp provides sender anonymity (See Section~\ref{anonymity-definition}) for a large number of Internet users. 
%As shown in Figure~\ref{fig:landmarks}, although the destination of each flow is known, the source information is replaced and traffic patterns are normalized at each landmark AS to provide sender anonymity. Additionally, the path length and location of each AS in a particular path is concealed in our protocol.


%\hcomment{I'm not sure how we can differentiate with LAP, here! Maybe we can say that our extended solution is supposed to have sender and receiver anonymity?}


%\item \textbf{Lightweight}: Most competing proposals rely heavily on  cryptographic operations performed at line speed on routers~\cite{lap,hornet}.  We identified the lack of support for such cryptographic operations in network equipment as a major impediment for deployment of network-level anonymity systems.  In our approach, however, we attain basic privacy properties without weighing down routing protocol routines in the data-plane with cryptographic overhead. Therefore, \protocolsp is a lightweight solution. In particular, we prototype our design on programmable hardware switches, optimized to run at the core of the Internet~\cite{barefoot}. Moreover, \protocolsp does not require carrying the entire forwarding state in packet headers (unlike LAP~\cite{lap}); thus, headers are of fixed size. This property makes the overhead of header processing at each border router constant size and independent of the number of participating ASes. Also, as opposed to HORNET~\cite{hornet}, \protocolsp does not require any prior knowledge of ASes along the path from source to destination. 

%\item \textbf{Deployable Solution}: \protocolsp is incrementally deployable and is compatible with existing Internet protocols, unlike other existing solutions~\cite{lap,dovetail,hornet}. Thus, \protocolsp brings sender anonymity to all users of a service provider, with no need for modifications on the clients' side and no changes in how most common Internet protocols operate, making our design easily deployable. Furthermore we prototype \protocolsp using state-of-the-art Software Defined Networking (SDN) technology~\cite{openflow} and to our knowledge, \protocolsp is the first SDN privacy enhancing solution in the context of inter-domain anonymity.



%\item \textbf{Multi-phased Deployment}:  \protocolsp deployment comprises of multiple stages. In the first stage, we provide sender anonymity through source information rewriting. Then, we extend \protocolsp to provide receiver anonymity, using source-controlled routing or pathlet routing~\cite{pathlet}. Our third stage is where different landmarks can coordinate, enabling asymmetric landmarks. Each stage, increases the cost of investment and coordination on service providers, but the set of features provided by \protocolsp expands, raising the anonymity bar.




%\end{itemize}





==> paper-07-disc-cgn.tex <==
\subsection{Comparison to Carrier-grade NAT}
%Network address translation (NAT)~\cite{natRFC} have been used widely used to work around IPv4 address exhaustion.


Faced with having fewer IPv4 addresses than the number of end hosts they have to serve, service providers have started deploying carrier-grade NATs (CGNs), across their networks. 
CGNs allow a small pool of public IPv4 addresses to be shared among many hosts and customers, by placing the NAT logic on a service provider's access network, rather than the subscribe edge, where NATs were traditionally located.



% There are a number of best practices around designing CGNs and protocols that interact with them~\cite{cgnReqRFC} and studies have shown the result of these practices in different providers~\cite{cgnStudy}. Some of the methods \protocolsp uses for DoS mitigation such as ingress filtering~\cite{ingressFilter}, TCP/UDP timeout are techniques shared between \protocolsp and CGN. 


% Therefore, CGN shifts the NAT function from the customer premises to the service provider network. There are a number of challenges the CGNs face, some of which are reported in~\cite{cgnReport}.  
%For instance, the number of simultaneous connections for different applications will be limited by a CGN due to port limitation. Also, CGNs must remain compatible with customer-premises equipment (CPE) deployed to perform customer-side NAT.






CGNs and \protocolsp share a number of similarities. For instance, they both perform source address rewriting and face scalability challenges such as maintaining the memory used for flow mapping. However, we argue these two technologies are fundamentally different in at least three aspects. 
 
 \emph{(i) Motivation}: CGNs are designed to address the problem of IPv4 exhaustion, whereas the goal of \protocolsp  is anonymity and unlinkability. Therefore, flow mappings are usually logged in CGNs\footnote{Service providers running CGNs are strongly encouraged to log the mapping to address abuses and requests from law enforcement~\cite{ipSharingRFC}.}, as opposed to \protocol, which only keeps mappings in memory and flushes them periodically.


 \emph{(ii) Mechanism}: 
Even though, both CGNs and \protocolsp generate flow mappings on the first packet of a flow, in the context of CGNs, flow mappings are not required to be secure. Thus, significant number of CGN vendors deploy port allocation strategies that preserve the original port address or increment it sequentially~\cite{cgnStudy}. On the other hand, \protocolsp mappings should be hard to invert and should not leak information resulting in either de-anonymization of flows or linking multiple flows belonging to the same user or application.
 Also, \emph{arbitrary pooling}, i.e., randomized selection of external public IP addresses assigned to flows, is mandatory in \protocol, whereas, study of CGNs show that only  21\% of them perform arbitrary pooling~\cite{cgnStudy}. 
Lastly, the default timeouts of flows in our design is different from CGNs, because a \protocolsp router not only obfuscates flows originating from its AS, but all flows transiting its network, potentially handling more flows than a CGN\footnote{If an AS decides to forgo obfuscating transiting flows, it loses the mixing advantage that transit traffic  provides.% to hide which flows belong to a particular ISP.
}.



% CGNs only perform IP and port rewriting. We change other fields too.
%No hairpinning, 
 
 
 \emph{(iii) Implications}: 
A major difference of \protocolsp echo system is that it does not require NAT traversal mechanisms, such as ICE or TCP/UDP hole punching, since we only obfuscate upstream flows. Also, as noted above, the different timeouts used in our design overrides the requirements designated for applications written for a CGN-enabled network~\cite{cgnReqRFC}, dictating new timing requirements for applications based on TCP or UDP. 
Finally, complicated by the fact that each landmark adds a layer of obfuscation,  abuse handling and DoS mitigation in \protocolsp is more challenging, as it is harder to identify the source of attacks. \protocolsp needs stricter control at the edges of the network, where abuses can be mitigated using ingress filtering~\cite{ingressFilter}, to protect infrastructures closer to the core.









%However, there are major differences between CGNs and \protocol. Primarily, \protocolsp does not act as a multiplexer of internal destinations and, thus, does not impose the kind of restriction that classical NATs place on network endpoints behind a NAT. For instance, in our design, an outside entity can use the address of a server located in a landmark AS directly to access the server. In fact, we argue there needs to be enough IP addresses allocated to individual hosts, with the caveat that we must make sure that no traffic correlation attacks can happen as a result of this design. Furthermore, \protocolsp explicitly mandates that service providers do not log the mapping between internal endpoint as opposed to CGNs.


%Another important distinction between CGNs and \protocolsp is that the mappings between flows and identifiers can only be reversed by the party holding the hash keys, whereas in CGNs the mapping (session outbound ports) are either deterministic or mostly predictable and as shown previously it can be used to link sessions of users, especially in the case of permissive (full cone) NAT which is quite prevalent in design of GCNs~\cite{cgnStudy}.



%\hcomment{Also, the mapping happens over a much bigger space, the tag is no longer just the port number(16 bit space), so it might not be performance-wise to iterate through all of it. Maybe discuss how long it will take to do it for 32 bit tags or }



